Understanding Large-Language Model (LLM)-powered Human-Robot Interaction

Large-language models (LLMs) hold significant promise in improving human-robot interaction, offering advanced conversational skills and versatility in managing diverse, open-ended user requests in various tasks and domains. Despite the potential to transform human-robot interaction, very little is known about the distinctive design requirements for utilizing LLMs in robots, which may differ from text and voice interaction and vary by task and context. To better understand these requirements, we conducted a user study (n = 32) comparing an LLM-powered social robot against text- and voice-based agents, analyzing task-based requirements in conversational tasks, including choose, generate, execute, and negotiate. Our findings show that LLM-powered robots elevate expectations for sophisticated non-verbal cues and excel in connection-building and deliberation, but fall short in logical communication and may induce anxiety. We provide design implications both for robots integrating LLMs and for fine-tuning LLMs for use with robots.

==> figure_godspeed.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/task_embodiment_godspeed_satisfaction.pdf}
  \caption{Boxplots with data points overlaid on anthropomorphism, animacy, likeability, and perceived intelligence. Tasks: (N)egotiate, (G)enerate, (C)hoose, (E)xecute; Embodiment: (T)ext, (V)oice, (R)obot. Due to high variance in data, no significant difference was found.}
  \label{app:godspeed}
\end{figure*}

==> figure_input_and_failure.tex <==
\begin{figure*}[t]
  \begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/figures_input.png}
    \caption{Total Input Tokens}
    \label{fig:inputs}
  \end{subfigure}%
  \begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/figures_failures.png}
    \caption{Total Failures}
    \label{fig:failures}
  \end{subfigure}
  \caption{Boxplots with data points overlaid on number of input tokens in the user prompt and number of failures occurred during the task. When users interacted with the text agent, there were no failures. We plotted by task, embodiment, and task$\ast$embodiment. Horizontal lines indicate significant pairwise comparisons with Tukey's HSD ($p < 0.05^{\ast}$, $p < 0.01^{\ast\ast}$, $p < 0.001^{\ast\ast\ast}$). Tasks: (N)egotiate, (G)enerate, (C)hoose, (E)xecute; Embodiment: (T)ext, (V)oice, (R)obot}
  \label{fig:input and failure}
\end{figure*}

==> figure_mcgrath.tex <==

\begin{figure}[!h]
    \centering
    \begin{tikzpicture}[scale=0.7]
  % Define the center of the circle
        \coordinate (center) at (0,0);
  
  % Draw the circle
        \draw (center) circle (3cm);

  % Add lines to separate the sections
        \draw (center) -- (45:3cm);
        \draw (center) -- (135:3cm);
        \draw (center) -- (225:3cm);
        \draw (center) -- (315:3cm);
  
  % Add text to the four quadrants
        \node at (90:2cm) {Generate};
        \node at (0:2cm) {Execute};
        \node at (270:2cm) {Negotiate};
        \node at (180:2cm) {Choose};

        % Add x and y axes
        \draw[<->] (-2.5,-3.5) node[left] {$cognitive$} -- (2.5,-3.5) node[right] {$behavorial$};
        \draw[<->] (3.5,-2.5) node[below] {$conflict$} -- (3.5,2.5) node[above] {$cooperation$};
    \end{tikzpicture}
    \caption{McGrath's Circumplex of Group Tasks}
    \label{fig:Mcgrath}
\end{figure}

==> figure_quant.tex <==
% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=\linewidth]{figures/task_embodiment_godspeed_satisfaction.png}
%   \caption{Boxplots with data points overlaid on perceived safety, satisfaction, total input tokens, and total failures. For each item, we plotted by ``embodiment'' and ``task grouped embodiment.'' Horizontal lines indicate significant pairwise comparisons with Tukey's HSD ($p < 0.05^{\ast}$, $p < 0.01^{\ast\ast}$, $p < 0.001^{\ast\ast\ast}$)}
%   \label{fig:quant}
% \end{figure*}

% \begin{figure}[htp]
%     \begin{subfigure}{\columnwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/input_failure.png}
%         %\vspace{-1em}
%         %\caption{Input length and Number of Failures}
%         \label{fig:input_failure}
%     \end{subfigure}
    
%   \begin{subfigure}{\columnwidth}
%     \centering
%     \includegraphics[width=\linewidth]{figures/satisfaction.png}
%     %\vspace{-1em}
%     %\caption{Users Perception and Satisfaction}
%     \label{fig:godspeed_satisfaction}
%   \end{subfigure}%
%   %\vspace{-1em}
%   \caption{Boxplots with data points overlaid on perceived safety, satisfaction, total input tokens, and total failures. For each item, we plotted by ``embodiment'' and ``task grouped by embodiment.'' Tasks: (N)egotiate, (G)enerate, (C)hoose, (E)xecute. Embodiment: (T)ext, (V)oice, (R)obot. Horizontal lines indicate significant pairwise comparisons with Tukey's HSD ($p < 0.05^{\ast}$, $p < 0.01^{\ast\ast}$, $p < 0.001^{\ast\ast\ast}$).}
%   \label{fig:quant}
% \end{figure}
